Thickness-dependent magnetic properties and strain-induced orbital magnetic moment in SrRuO3 thin films

Thin films of the ferromagnetic metal SrRuO3 (SRO) show a varying easy magnetization axis depending on the epitaxial strain and undergo a metal-to-insulator transition with decreasing film thickness. We have investigated the magnetic properties of SRO thin films with varying thicknesses fabricated on SrTiO3(001) substrates by soft x-ray magnetic circular dichroism (XMCD) at the Ru M2,3 edge. Results have shown that, with decreasing film thickness, the film changes from ferromagnetic to non-magnetic around 3monolayer thickness, consistent with previous magnetization and magneto-optical Kerr effect measurements. The orbital magnetic moment perpendicular to the film was found to be ~ 0.1{\mu}B/Ru atom, and remained nearly unchanged with decreasing film thickness while the spin magnetic moment decreases. Mechanism for the formation of the orbital magnetic moment is discussed based on the electronic structure of the compressively strained SRO film.

==> common.tex <==
\usepackage{xspace}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{siunitx}
\usepackage{abbrevs}
\usepackage{etoolbox}

%\usepackage{todonotes}
%\hypersetup{unicode}

\makeatletter
\def\and@for#1#2#3#4{%
\@tempcnta=\z@% ここでカウンタをクリア
\@tempcntb=\z@% ここでカウンタをクリア
\@for\member:=#1\do{\advance\@tempcnta\@ne}% メンバー数の計算
\@for\member:=#1\do{\advance\@tempcntb\@ne}% メンバー数の計算
\ifnum\@tempcntb>1\relax% 最後から二つ目ならば `\member and'
#3\else%
#2\fi% \end{ifnum}
\ \@for\member:=#1\do{% 実際の処理
\ifnum\@tempcnta>2\relax% 2 以上ならばカンマ付
\ref{#4:\member},\ \else%
\ifnum\@tempcnta=2\relax% 最後から二つ目ならば `\member and'
\ref{#4:\member}\relax%
\ifnum\@tempcntb>2\relax% 最後から二つ目ならば `\member and'
,\fi% \end{ifnum}
\ and\ \else%
\ifnum\@tempcnta=1\relax% 最後の一つなら直接出力
\ref{#4:\member}\fi% \end{ifnum}
\fi% \end{ifnum}
\fi% \end{ifnum}
\advance\@tempcnta\m@ne% カウンタを一つ減少させる
}% \end{for}
}%
\let\andforr\and@for
\makeatother

% \newenvironment{FinishReview}{%
% % \color{BrickRed}%
% \color{Gray}%
% }{}
% 
% \newenvironment{PlzReviewFujimori}{%
% \color{OliveGreen}%
% }{%
% }
% 
% \newenvironment{PlzReviewYoshida}{%
% \color{Blue}%
% }{}
% 
% \newenvironment{ReplyFix}{%
% \color{Black}
% }{}
% \newcommand{\ReplyFixText}[1]{\textcolor{Black}{#1}}
% 
% \newenvironment{ReplyFixPlzReview}{%
% \color{Red}
% }{}
% \newcommand{\ReplyFixPlzReviewText}[1]{\textcolor{Red}{#1}}
% 
% \newcommand{\ReplyNote}[1]{\todo[noline, color=Lavender]{#1}}
% \newcommand{\ReplyFig}[1]{\relax%
% \fcolorbox{BrickRed}{white}{#1}\relax%
% }

\newcommand{\BSTO}[0]{(Ba,Sr)TiO$_3$\xspace}
\newcommand{\CSRO}[0]{Ca$_{1-x}$Sr$_x$RuO$_{3}$\xspace}
\newcommand{\LSTO}[0]{La$_{1-x}$Sr$_{x}$TiO$_3$\xspace}
\newcommand{\LSMO}[0]{La$_{0.6}$Sr$_{0.4}$MnO$_3$\xspace}
\newcommand{\NSTO}[0]{Nb:SrTiO$_3$\xspace}
% \newcommand{\STO}[0]{SrTiO$_3$\xspace}
\newcommand{\STO}[0]{SrTiO$_3$}
\newcommand{\STRO}[0]{SrTi$_{1-x}$Ru$_x$O$_3$\xspace}
\newcommand{\TiOtwo}[0]{TiO$_2$\xspace}
\newcommand{\LTO}[0]{LaTiO$_3$\xspace}
\newcommand{\GFO}[0]{GdFeO$_3$\xspace}
\newcommand{\SLTO}[0]{Sr$_{1-x}$La$_{x}$TiO$_3$\xspace}
\newcommand{\LCVO}[0]{La$_{1-x}$Ca$_{x}$VO$_3$\xspace}
\newcommand{\LVO}[0]{LaVO$_3$\xspace}
\newcommand{\CVO}[0]{CaVO$_3$\xspace}
\newcommand{\SrO}[0]{SrO\xspace}
\newcommand{\LaSrO}[0]{La$_{1-x}$Sr$_x$O\xspace}
\newcommand{\LAO}[0]{LaAlO$_3$\xspace}
\newcommand{\LaO}[0]{LaO\xspace}
\newcommand{\AlOtwo}[0]{AlO$_2$\xspace}

\newcommand{\hn}[0]{$h\nu$\xspace}
\newcommand{\muB}[0]{$\mu_\text{B}$\xspace}
%\newcommand{\muB}[0]{\begin{ReplyFix}$\mu_\text{B}$\end{ReplyFix}\xspace}
%\newcommand{\muZero}[0]{\begin{ReplyFix}$\mu_\text{0}$\end{ReplyFix}\xspace}

\newcommand{\Exsitu}[0]{\textit{Ex situ}\xspace}
\newcommand{\exsitu}[0]{\textit{ex situ}\xspace}
\newcommand{\Insitu}[0]{\textit{In situ}\xspace}
\newcommand{\insitu}[0]{\textit{in situ}\xspace}
\newcommand{\etal}[0]{\textit{et al.}\xspace}

% \newcommand{\orbit}[1]{{\textsl #1}}
\newcommand{\orbit}[1]{$#1$}
\newcommand{\valence}[1]{{$^{#1}$}}



\newcommand{\XAS}[0]{X-ray absorption spectroscopy\xspace}
\newcommand{\XMCD}[0]{X-ray magnetic circular dichroism\xspace}

\newcommand{\figl}[1]{\label{fig:#1}}
\newcommand{\figr}[1]{\andforr{#1}{Fig.}{Figs.}{fig}}
\newcommand{\figurer}[1]{\andforr{#1}{Figure}{Figures}{fig}}
\newcommand{\tbll}[1]{\label{tbl:#1}}
\newcommand{\eqnl}[1]{\label{eqn:#1}}
%\newcommand{\eqnr}[1]{\andforr{#1}{Eq.}{Eqs.}{eqn}}
\newcommand{\CO}[0]{(Color online)\xspace}

\newcommand{\UTPhys}[0]{Department of Physics, University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\UTChem}[0]{Department of Applied Chemistry, The University of Tokyo, Bunkyo-ku, Tokyo 113-8656, Japan}
\newcommand{\UTCmpS}[0]{Department of Complexity Science and Engineering, The University of Tokyo, Kashiwa, Chiba 277-0882, Japan}
\newcommand{\PFIMSS}[0]{Photon Factory, IMSS, High Energy Accelerator Research Organization, Tsukuba, Ibaraki 305-0801, Japan}
\newcommand{\JAEA}[0]{Quantum Beam Science Directorate, Japan Atomic Energy Agency, Sayo, Hyogo 679-5148, Japan}

\newabbrev{\FermiLevel}{Fermi level ($E_\text{F}$)}[$E_\text{F}$]
%\newcommand{\EF}[0]{\begin{ReplyFix}\protect\FermiLevel\end{ReplyFix}}
\newcommand{\EF}[0]{\protect\FermiLevel\protect\xspace}
%\newcommand{\EF}[0]{\FermiLevel\let\maybe@space@\xspace}
% \protect\EF
\robustify{\EF}
% \DeclareRobustCommand{\EF}

% \newcommand{\SRO}[0]{SrRuO$_3$\xspace}
\newcommand{\SRO}[0]{SrRuO$_3$}
% \newcommand{\SROSn}[0]{SRO\xspace}
% \newcommand{\SROLn}[0]{SrRuO$_3$\xspace}
% \newabbrev{\SRO}{\SROLn (\SROSn)}[SRO]
% \robustify{\SRO}


\makeatletter
\renewcommand\maybe@space@{%
% \@tempswatrue % <= this is in the original
\maybe@ictrue % <= this is new
\expandafter   \@tfor
\expandafter \reserved@a
\expandafter :%
\expandafter =%
\nospacelist
\do \t@st@ic
% \if@tempswa % <= this is in the original
\ifmaybe@ic % <= this is new
\space
\fi
}
\makeatother

